The Ruble Collapse in an Online Marketplace: Some Lessons for Market Designers

The sharp devaluation of the ruble in 2014 increased the real returns to Russians from working in a global online labor marketplace, as con- tracts in this market are dollar-denominated. Russians clearly noticed the opportunity, with Russian hours-worked increasing substantially, primarily on the extensive margin -- incumbent Russians already active were fairly inelastic. Contrary to the predictions of bargaining models, there was little to no pass-through of the ruble price changes in to wages. There was also no evidence of a demand-side response, with buyers not posting more "Russian friendly" jobs, suggesting limited cross-side externalities. The key findings -- a high extensive margin elasticity but low intensive margin elasticity; little pass-through into wages; and little evidence of a cross-side externality -- have implications for market designers with respect to pricing and supply acquisition.

==> tables/job_opening_wages_and_hiring.tex <==

\begin{table}[!htbp] \centering 
  \caption{Effects of the ruble collapse on per-vacancy measures of wage bidding and hiring} 
  \label{tab:job_opening_wages_and_hiring} 
\small 
\begin{tabular}{@{\extracolsep{5pt}}lccc} 
\\[-1.8ex]\hline 
\hline \\[-1.8ex] 
 & \multicolumn{3}{c}{\textit{Dependent variable:}} \\ 
\cline{2-4} 
\\[-1.8ex] & Wages & Any Russian hires? & Any hires? \\ 
\\[-1.8ex] & (1) & (2) & (3)\\ 
\hline \\[-1.8ex] 
 log(Price):bands(1.8e-06,0.1] & 0.085 & 0.006 & $-$0.162 \\ 
  & (0.169) & (0.023) & (0.150) \\ 
  & & & \\ 
 log(Price):bands(0.1,0.25] & 0.090 & 0.009 & $-$0.171 \\ 
  & (0.166) & (0.022) & (0.147) \\ 
  & & & \\ 
 log(Price):bands(0.25,0.5] & 0.083 & 0.008 & $-$0.175 \\ 
  & (0.163) & (0.022) & (0.145) \\ 
  & & & \\ 
 log(Price):bands(0.5,0.75] & $-$0.014 & 0.005 & $-$0.319$^{**}$ \\ 
  & (0.163) & (0.022) & (0.145) \\ 
  & & & \\ 
 log(Price):bands(0.75,1] & 0.103 & 0.045$^{**}$ & $-$0.240$^{*}$ \\ 
  & (0.164) & (0.022) & (0.145) \\ 
  & & & \\ 
\hline \\[-1.8ex] 
Observations & 303,104 & 303,104 & 303,104 \\ 
R$^{2}$ & 0.251 & 0.009 & 0.006 \\ 
Adjusted R$^{2}$ & 0.251 & 0.008 & 0.006 \\ 
\hline 
\hline \\[-1.8ex] 
\end{tabular}
\\
\begin{minipage}{0.95 \textwidth}
{\footnotesize \emph{Notes}:
This table reports regressions on vacancy level outcomes on changes in the price of the USD (measured in rubles) and its interaction with a measure of how compatible a vacancy is to Russians. 
The sample consists of all vacancies posted using the period covered by the country-week panel. 
The outcome in Column~(1) is the log number of applications received by vacancy.
The outcome in Column~(2) is the log average wage of the applicants interviewed by the employer.
The outcome in Column~(3) is an indicator for whether the employer hired anyone.
The main independent variable is $p_t$ interacted with the Russian compatatibility score bands, which is the price of 1 USD, measured in Russian roubles at the start of week $t$.
The measure $s_{i}$, which is the predicted fraction of applicants that would be Russian based the predictions from a model, using historical data from the marketplace.  
\starlanguage}
\end{minipage}
\end{table}

